Adjoint Complement to the Universal Momentum Law of the Wall

The paper is devoted to an adjoint complement to the universal Law of the Wall (LoW) for fluid dynamic momentum boundary layers. The latter typically follows from a strongly simplified, unidirectional shear flow under a constant stress assumption. We first derive the adjoint companion of the simplified momentum equation, while distinguishing between two strategies. Using mixing-length arguments, we demonstrate that the frozen turbulence strategy and a LoW-consistent (differentiated) approach provide virtually the same adjoint momentum equations, that differ only in a single scalar coefficient controlling the inclination in the logarithmic region. Moreover, it is seen that an adjoint LoW can be derived which resembles its primal counterpart in many aspects. The strategy is also compatible with wall-function assumptions for prominent RANS-type two-equation turbulence models, which ground on the mixing-length hypothesis. As a direct consequence of the frequently employed assumption that all primal flow properties algebraically scale with the friction velocity, it is demonstrated that a simple algebraic expression provides a consistent closure of the adjoint momentum equation in the logarithmic layer. This algebraic adjoint closure might also serve as an approximation for more general adjoint flow optimization studies using standard one- or two-equation Boussinesq-viscosity models for the primal flow. Results obtained from the suggested algebraic closure are verified against the primal/adjoint LoW formulations for both, low- and high-Re settings. Applications included in this paper refer to two- and three-dimensional shape optimizations of internal and external engineering flows. Related results indicate that the proposed adjoint algebraic turbulence closure accelerates the optimization process and provides improved optima in comparison to the frozen turbulence approach.

==> tex/loglaw_variations.tex <==
\section{Kommentare LoW für turbulente Strömungen}

\subsection{Primale Wandfunktionen}
Der primale Zweibereichsansatz für die normierte Scherspannung
$\tau_e / \rho = const. = U_\tau^2 $ lautet
\begin{alignat}{2}
y^+ < {Y^+}:& \qquad
\nu \frac{\partial u}{\partial y} = U_{\tau}^2 \qquad \to \qquad 
\frac{\partial u}{\partial y} = 
\frac{U_{\tau}^2}{\nu}  ,
\label{eq1}
\\
y^+ \ge {Y^+}:&\qquad
 (\kappa y)^2 \left(\frac{\partial u}{\partial y}\right)^2 = U_{\tau}^2 \qquad \to \qquad 
\frac{\partial u}{\partial y} =
\frac{U_{\tau}}{\kappa y} =
\frac{U_{\tau}^2}{\nu} \left( \frac{1}{\kappa} 
\frac{1}{y^+} \right) \, .
\label{eq2}
\end{alignat}
Faktisch knickt die Steigung daher um den Faktor 
$(\kappa y^+)^{-1}$ mit Eintritt in den logarithmischen Bereich.
Ferner lautet die effektive bzw. turbulente Zähigkeit im log-Bereich
$$
 \nu_{log} = 
\nu \, \kappa y^+ =  U_\tau \; \kappa y 
$$
Das turbulente Geschwindigkeits- und Längenmaß lautet somit
$$
V_{turb} = U_\tau (=| \overline{u'v'}|) \; , \qquad
L_{turb} = \kappa y
$$
Dies findet man auch aus $k-\epsilon$ und allen anderen TM-Strategien, wenn man die Wandfunktionen für die Turbulenzmodellparameter einsetzt, z.B. für $k$ und $\epsilon$
\begin{alignat}{2}
k_{log} = \frac{U_\tau^2}{\sqrt{c_\mu}} \, , \qquad 
\epsilon_{log} = \frac{U_\tau^3}{\kappa y}
\label{eq3}
\\
 \nu_{log} = c_\mu \frac{k^2}{\epsilon} = U_\tau \; \kappa y 
 \, .
\label{eq4}
\end{alignat}
Man erkennt: {\bf Alles parametrisiert mit der Wandschubspannung
$U_\tau$!} Ferner kann man für die untersuchte, sehr einfache Strömung ein sog. Nullgleichungs-TM bzw. algebraisches TM verwenden, bei dem $\nu_t = U_\tau \, \kappa y$ gesetzt wird, wobei man $U_\tau$ aus der Wandschubspannung iterativ berechnet.

\subsection{Variation der Primalen Wandfunktionen}
Die Variation der Schubspannung ist trivial und lautet
\begin{equation}
\delta \tau_e/\rho = 2 U_\tau \, \delta U_\tau
\label{eq:5}
\end{equation}
Die Beziehung wird nat. auch für die log-law-Ansätze und allg. Wandfunktionen bestätigt. Für den algeraischen Ansatz findet man sofort
\begin{equation}
\tau_e/\rho = (U_\tau \, \kappa y) \frac{\partial u}{\partial y} =  (U_\tau \, \kappa y) \, \frac{U_\tau
}{\kappa y} = U_\tau^2 
\label{eq:6}
\end{equation}
und damit wieder (\ref{eq:5}). Wenn man hierin den Beitrag der turbulenten Zähigkeit einfriert, {\bf halbiert sich die Variation}
\begin{equation}
\delta \tau_e/\rho = \overline{(U_\tau \, \kappa y)} \delta \left(\frac{\partial u}{\partial y}\right) =  (U_\tau \, \kappa y) \, \frac{\delta U_\tau
}{\kappa y} = (\delta U_\tau) \, U_\tau 
\label{eq:7}
\end{equation}
Analog liefert die Variation der turbulenten Zähigkeit die zweite Hälfte, d.h. $\delta \nu_{log} = \kappa y \, \delta U_\tau$ und damit $\delta v_{log} \, \overline{\partial u/\partial y} = (\delta U_\tau) U_\tau $

\noindent 
Das Ergebnis wird auch durch die 2-Glg.-Modelle bestätigt, wenn man Wandfunktionen benutzt. Für das $k-\epsilon$ Modell findet man z.B. 
\begin{equation}
\delta \nu_{log} = c_\mu \frac{k}{\epsilon} \left( 2 \delta k -
 \frac{k}{\epsilon} \delta \epsilon
\right) 
\label{eq:8}
\end{equation}
Setzt man hierin die log-Beziehungen $k/\epsilon= \kappa y/U_\tau /\sqrt{c_\mu}$ sowie $\delta k = 2(\delta U_\tau) U_\tau /\sqrt{c_\mu}
$ bzw.
$\delta \epsilon = 3(\delta U_\tau) U_\tau^2/(\kappa y)$ ein, dann ergibt sich erneut
\begin{equation}
\delta \nu_{log} = \sqrt{c_\mu} \frac{\kappa y}{U_\tau} 
\left( 4 (\delta U_\tau) U_\tau - 3 (\delta U_\tau) U_\tau
\right) = \kappa y (\delta U_\tau)
\label{eq:9}
\end{equation}

\subsection{Duale Beziehungen}
Der duale Zweibereichsansatz für die normierte Scherspannung
$\hat \tau_e / \rho = const. = U_\tau^2 $ kann vom primalen Ansatz im Grundsatz übernommen werden. Wenn man dieo.g. log-Beziehungen einsetzt erhält man 
\begin{alignat}{2}
y^+ < {Y^+}:& \qquad
\nu \frac{\partial \hat u}{\partial y} = \hat U_{\tau}^2 \qquad \to \qquad 
\frac{\partial \hat u}{\partial y} = 
\frac{\hat U_{\tau}^2}{\nu}  ,
\label{eq10}
\\
y^+ \ge {Y^+}:&\qquad
 2 (\kappa y)^2 \frac{\partial u}{\partial y}
 \frac{\partial \hat u}{\partial y} = \hat U_{\tau}^2 \qquad \to \qquad 
\frac{\partial \hat u}{\partial y} =
\frac{\hat U_{\tau}^2}{2 \, U_\tau \, \kappa y} =
\frac{\hat U_{\tau}^2}{\nu} \left( \frac{1}{2 \, \kappa} 
\frac{1}{y^+} \right) \, .
\label{eq11}
\end{alignat}
Faktisch knickt die Steigung in adjungierten Fall um den Faktor 
$(2 \kappa y^+)^{-1}$ mit Eintritt in den logarithmischen Bereich.
Ferner verdoppelt sich die effektive bzw. turbulente Zähigkeit im Vergleich zur primalen Lösung für den log-Bereich
$$
 \hat \nu_{log} = 
2 \, \nu \, \kappa y^+ =  2 \, U_\tau \; \kappa y =
 2\, \nu_{log}
$$
Das turbulente Geschwindigkeits- und Längenmaß lautet somit
$$
\hat V_{turb} = 2 U_\tau (=| \overline{u'v'}|) \; , \qquad
L_{turb} = \kappa y
$$
Man könnte  schließen, dass eine adjungierte TM mit einem 4-fachen $k$ und einem 8-fachen $\epsilon$ verknüpft ist.

\section{Code-nahes adjungieren}

Wenn man anstelle von
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \hat{u} \frac{\mathrm{d}}{\mathrm{d} y} \left[ (\kappa \, y)^2 \left(\frac{\mathrm{d} u}{\mathrm{d} y}\right)^2 \right] + \hat{k} \left[k - \frac{U_\tau^2}{\sqrt{C_\mu}} \right] + \hat{\epsilon} \left[\epsilon - \frac{U_\tau^3}{\kappa y} \right] \right] \mathrm{d} y \, . 
\end{align}
die Wandfunktion $\epsilon= U_\tau^3/(\kappa y)= (k \sqrt{c_\mu})^{3/2}/(\kappa y)$ in den dritten Teil einsetzt, ergibt sich 
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \hat{u} \frac{\mathrm{d}}{\mathrm{d} y} \left[ (\kappa \, y)^2 \left(\frac{\mathrm{d} u}{\mathrm{d} y}\right)^2 \right] + \hat{k} \left[k - \frac{U_\tau^2}{\sqrt{C_\mu}} \right] + \hat{\epsilon} \left[\epsilon - \frac{(k \sqrt{C_\mu})^{3/2}}{\kappa y} \right] \right] \mathrm{d} y \, . 
\end{align}
Zerlegt man nun weiter den Ausdruck im ersten Teil einmal(!) durch  
$(\kappa y) \partial u/ \partial y = U_\tau = (k \sqrt{C_\mu})^{1/2} $
%$U_\tau^2 = U_\tau \cdot U_\tau = (\kappa y) \partial u/ \partial y \cdot (k \sqrt{c_\mu})^{1/2}  $
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \hat{u} 
        \frac{\mathrm{d}}{\mathrm{d} y}\left[ (\kappa \, y) \left(\frac{\mathrm{d} u}{\mathrm{d} y} \right) \cdot 
         (k \sqrt{c_\mu})^{1/2} \right] + \hat{k} \left[k - \frac{U_\tau^2}{\sqrt{C_\mu}} \right] + \hat{\epsilon} \left[\epsilon - \frac{(k \sqrt{C_\mu})^{3/2}}{\kappa y} \right] \right] \mathrm{d} y \, .
\end{align}
dann ergibt sich durch Variation
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \int_y \left[ \delta j_\mathrm{\Omega} +  \hat{u} 
         \frac{\mathrm{d}}{\mathrm{d} y} \left[ (\kappa \, y) \left(\frac{\mathrm{d} \delta u}{\mathrm{d} y} \right) \cdot 
         (k \sqrt{C_\mu})^{1/2} +
         (\kappa \, y) \left(\frac{\mathrm{d}  u}{\mathrm{d} y}\right)
          \delta k  \frac{C_\mu^{1/4}}{2 \sqrt{k}}
          \right] + \hat{k} \left[\delta k - 2 \frac{U_\tau}{\sqrt{C_\mu}} \delta U_\tau \right] + \hat{\epsilon} \left[\delta \epsilon - 
           \delta k \frac{3 \sqrt{k}  C_\mu^{1/4}}{2 \kappa y} \right] \right] \mathrm{d} y \, .
\end{align}
Da man im Rahmen der Wandfunktion $\delta U_\tau = (\kappa y) \, d \delta u / d y $ einsetzen kann, ergibt sich
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \int_y \left[ \delta j_\mathrm{\Omega} +  \hat{u} 
        \frac{\mathrm{d}}{\mathrm{d} y} \left[ (\kappa \, y) \left(\frac{\mathrm{d} \delta u}{\mathrm{d} y} \right) \cdot 
         (k \sqrt{C_\mu})^{1/2} +
         (\kappa \, y) \left(\frac{\mathrm{d}  u}{\mathrm{d} y}\right)
          \delta k  \frac{C_\mu^{1/4}}{2 \sqrt{k}}
          \right] + \hat{k} \left[\delta k - 2 \frac{U_\tau \kappa y}{\sqrt{C_\mu}} \frac{d \delta u}{dy}\right] + \hat{\epsilon} \left[\delta \epsilon - 
           \delta k \frac{3 \sqrt{k}  C_\mu^{1/4}}{2 \kappa y} \right] \right] \mathrm{d} y \, .
             \label{eq:h0}
\end{align}
 Die partielle Integration der 1. Klammer ergibt
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \oint \dots
        + \int_y \left[ \delta j_\mathrm{\Omega} - \frac{\mathrm{d \hat u}}{\mathrm{d} y}
         \left[ (\kappa \, y) \left(\frac{\mathrm{d} \delta u}{\mathrm{d} y} \right) \cdot 
         (k \sqrt{C_\mu})^{1/2} +
         (\kappa \, y) \left(\frac{\mathrm{d}  u}{\mathrm{d} y}\right)
          \delta k  \frac{C_\mu^{1/4}}{2 \sqrt{k}}
          \right] \right] dy  \nonumber \\  
          + \int_y \hat{k} \left[ \delta k - 2 \frac{U_\tau \kappa y}{\sqrt{C_\mu}}  \frac{d \delta u}{dy} \right] dy
 + \int_y \hat{\epsilon} \left[\delta \epsilon - \delta k \frac{3 \sqrt{k}  c_\mu^{1/4}}{2 \kappa y} \right] \mathrm{d} y \, .
  \label{eq:h1}
\end{align}
Erneute partielle Integration zweier Terme ergibt
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \oint \dots
        + \int_y \left[ \delta j_\mathrm{\Omega} - \delta k
        \left( 
         (\kappa \, y) \left(\frac{\mathrm{d}  u}{\mathrm{d} y}\right)
         \frac{\mathrm{d \hat u}}{\mathrm{d} y} \; 
         \frac{C_\mu^{1/4}}{2 \sqrt{k}}
        \right) \right] dy  
       + \int_y \delta u 
         \frac{\mathrm{d}}{\mathrm{d} y} 
         \left[ 
          (\kappa \, y)  (k \sqrt{C_\mu})^{1/2}  \, 
       \left( \frac{\mathrm{d} \hat u}{\mathrm{d} y} \right) 
          \right]  
       \nonumber \\  
         + \int_y \delta k 
         \left[ \hat{k} \right] dy
         + \int_y \delta u  \frac{\mathrm{d}}{\mathrm{d} y}  
         \left[ 2 \hat k \, \frac{U_\tau \kappa y}{\sqrt{C_\mu}} 
           \right] dy
  + \int_y \delta \epsilon [\hat{\epsilon}] dy -
   \int_y \delta k \left[  \hat{\epsilon} \, \frac{3 \sqrt{k}  
  c_\mu^{1/4}}{2 \kappa y} \right] \mathrm{d} y \, .
 \label{eq:h2}
\end{align}
Hieraus lassen sich die folgenden adjungierten WF-Gleichungen ableiten 
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \int_y \left[ \delta j_\mathrm{\Omega} +  \delta u \,
        \frac{\mathrm{d}}{\mathrm{d} y}  \left[\left(\frac{\mathrm{d} \hat u}{\mathrm{d} y}\right)
          (\kappa \, y)  \cdot  (k \sqrt{C_\mu})^{1/2} 
         +2\hat k \, \frac{U_\tau \kappa y}{\sqrt{C_\mu}} 
          \right]  + 
            \delta k \left[  \hat{k} -\hat{\epsilon}  \frac{3 \sqrt{k}  C_\mu^{1/4}}{2 \kappa y} -
            \frac{C_\mu^{1/4}}{2 \sqrt{k}} \, (\kappa \, y) \left(\frac{\mathrm{d}  u}{\mathrm{d} y}\right) \left(\frac{\mathrm{d} \hat u}{\mathrm{d} y}\right)
            \right] +
           \delta \epsilon \left[ \hat{\epsilon} \right]
           \right] \mathrm{d} y \, .
\end{align}
Setzt man in diesen Ausdruck wieder primale Ausdrücke ein, die alles als Funktion von $U_\tau$ formulieren, dann erhält man
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \delta u \,
        \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
        U_\tau \kappa \, y 
        \left(
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
         +  \frac{2\hat k}{\sqrt{C_\mu}} \right) 
          \right]  + 
             \delta k \left[  \hat{k} -\hat{\epsilon} \,  \frac{3 U_\tau }{2 \kappa y} -
             \frac{\sqrt{C_\mu}}{2} \,  \left(\frac{\mathrm{d} \hat u}{\mathrm{d} y}\right)
            \right] +
           \delta \epsilon \left[ \hat{\epsilon} \right]
           \right] \mathrm{d} y \, .
\end{align}
\begin{align}
    \hat{\epsilon} = 0 
    \quad \mathrm{and} \quad 
    \hat{k} =  \frac{\sqrt{C_\mu}}{2} \,  \left(\frac{\mathrm{d}  \hat u}{\mathrm{d} y} \right)
    \qquad \rightarrow \qquad
    \int_y \left[ 
    \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
       2 (U_\tau \kappa \, y) \; 
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
          \right] 
     \right] dy = 0 .
     \label{eq:result}
\end{align}
Man beachte, dass $\nu_t = U_\tau \kappa y$.

\subsubsection{Randintegrale}

Ich erhalte im Schritt von (\ref{eq:h0}) zu (\ref{eq:h1}) folgende Randterme
\begin{align}
    \oint \hat u \left[ 
    \frac{d \delta u}{dy} \; (\kappa y) (k \sqrt{C_\mu})^{1/2} + \delta k \; \frac{\kappa y }{2}
     \frac{du}{dy} \sqrt{\frac{C_\mu^{1/2}}{k}} \right]
    .
\end{align}
Setzt man hierin log-Beziehungen ein, dann ergibt sich
\begin{align}
    \oint \hat u \left[ 
    \frac{d \delta u}{dy} \; (U_\tau \kappa y) + \delta k \; \frac{\sqrt{C_\mu} }{2}
     \right]
     \label{eq:wasnun}
    .
\end{align}
Ergänzend ergibt sich bei den Umformungen von  (\ref{eq:h1}) zu (\ref{eq:h2})
\begin{align}
   - \oint  \delta u \left[ 
    \frac{d \hat u}{dy} \; (\kappa y) (k \sqrt{C_\mu})^{1/2} + 
    2 \hat k  \frac{U_\tau \kappa y}{\sqrt{C_\mu}}
     \right]
    .
\end{align}
Setzt man auch hier log-Beziehungen ein, erhält man
\begin{align}
   - \oint  \delta u \left[ U_\tau \kappa y \left(
    \frac{d \hat u}{dy} \;  + 
      \frac{2 \hat k}{\sqrt{C_\mu}} \right) 
     \right]
    .
\end{align}
Unterstellt man, dass die WF-Beziehung (\ref{eq:result}) auch an der Wand gilt, ergibt der letzte Ausdruck einen Zugang zur bekannten Sensitivität
\begin{align}
   - \oint  \delta u \left[ 2 U_\tau \kappa y \
    \frac{d \hat u}{dy} \right]
    \qquad {\rm mit} \qquad \delta u = - \frac{du}{dy} \delta y \quad {\rm und} \quad \nu_t = U_\tau \, \kappa y
    .
\end{align}
Für die Zielfunktion x-Kraft auf die Wand resultieren aus $j_\Gamma= \nu_\mathrm{eff} du/dy = (U_\tau \kappa y) du/dy$ die folgenden Variationsbeiträge
\begin{align}
    \oint  \delta U_\tau (\kappa y) \frac{du}{dy} + 
    \oint (U_\tau \kappa y)  \frac{d \delta u}{dy}
    .
    \label{eq:dasnun}
\end{align}
Wir verwenden die Variation der $k$-WF, d.h. $\delta k = 2 U_\tau \delta U_\tau /\sqrt{C_\mu}$, und notieren anstellen von (\ref{eq:dasnun}) 
 \begin{align}
    \oint  \delta k \frac{(\kappa y)}{U_\tau} \, \frac{\sqrt{C_\mu}}{2} \frac{du}{dy} + 
    \oint (U_\tau \kappa y)  \frac{d \delta u}{dy}
    .
    \label{eq:dasnun2}
\end{align}
Setzt man in die Gleichung (\ref{eq:dasnun2}) erneut log-Beziehungen ein, dan ergibt sich
\begin{align}
    \oint  \delta k \, \frac{\sqrt{C_\mu}}{2}  + 
    \oint (U_\tau \kappa y)  \frac{d \delta u}{dy}
    .
    \label{eq:dasnun3}
\end{align}
Gleichung (\ref{eq:dasnun3}) und (\ref{eq:wasnun}) neutralisieren sich nur unter der (üblichen) adjungierten Wandrandbedingung 
$$
\hat u \equiv -1 \; !
$$

\subsection{Low-Re}
Anstelle von
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \hat{u} \frac{\mathrm{d}}{\mathrm{d} y} \left[ \nu  \left(\frac{\mathrm{d} u}{\mathrm{d} y}\right) \right] + \hat{k} \left[k \right] + \hat{\epsilon} \left[\epsilon - 2 \nu \frac{k}{y^2} \right] \right] \mathrm{d} y \, . 
\end{align}
erhält mE nach einigem hin und her
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \int_y \left[ \delta j_\mathrm{\Omega} +  \delta u \,
        \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
       \nu
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
          \right]  + 
             \delta k \left[  \hat{k} -\hat{\epsilon} \,  \frac{2 \nu }{y^2} 
            \right] +
           \delta \epsilon \left[ \hat{\epsilon} \right]
           \right] \mathrm{d} y \, .
\end{align}
\begin{align}
    \hat{\epsilon} = 0 
    \quad \mathrm{and} \quad 
    \hat{k} =  0
    \qquad \rightarrow \qquad
    \int_y \left[ 
    \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
      \nu  \; 
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
          \right] 
     \right] dy = 0 .
\end{align}
Setzt man alternativ im Primalen 
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \hat{u} \frac{\mathrm{d}}{\mathrm{d} y} \left[ \nu  \left(\frac{\mathrm{d} u}{\mathrm{d} y}\right) \right] + \hat{k} \left[\frac{d k}{dy} \right] + \hat{\epsilon} \left[\epsilon - 2 \nu \frac{k}{y^2} \right] \right] \mathrm{d} y \, . 
\end{align}
erhält mE nach einigem hin und her
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \int_y \left[ \delta j_\mathrm{\Omega} +  \delta u \,
        \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
       \nu
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
          \right]  - 
             \delta k \left[  \frac{d\hat{k}}{dy} + \hat{\epsilon} \,  \frac{2 \nu }{y^2} 
            \right] +
           \delta \epsilon \left[ \hat{\epsilon} \right]
           \right] \mathrm{d} y \, .
\end{align}
\begin{align}
    \hat{\epsilon} = 0 
    \quad \mathrm{and} \quad 
    \frac{d\hat{k}}{dy} =0 
    \qquad \rightarrow \qquad
    \int_y \left[ 
    \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
      \nu  \; 
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
          \right] 
     \right] dy = 0 .
\end{align}
\subsection{Etwas ulkig ????????}
wird es wenn man exakt die folgende -- in Bezug auf $k$ hybride -- Version des primalen ansetzt. Dies enttarnt vermutlich Unsauberkeiten ...
\begin{align}
        L = j_\mathrm{\Gamma} + \int_y \left[ j_\mathrm{\Omega} +  \hat{u} 
        \frac{\mathrm{d}}{\mathrm{d} y} \left[ (\kappa \, y) \left(\frac{\mathrm{d} \delta u}{\mathrm{d} y} \right) \cdot 
         (k \sqrt{C_\mu})^{1/2} +
         (\kappa \, y) \left(\frac{\mathrm{d}  u}{\mathrm{d} y}\right)
          \delta k  \frac{C_\mu^{1/4}}{2 \sqrt{k}}
          \right] + \hat{k} \left[\frac{d \delta k}{dy} \right] + \hat{\epsilon} \left[\delta \epsilon - 
           \delta k \frac{3 \sqrt{k}  C_\mu^{1/4}}{2 \kappa y} \right] \right] \mathrm{d} y \, .
\end{align}
Man erhält mE nach einigem hin und her
\begin{align}
        \delta L = \delta j_\mathrm{\Gamma} + \int_y \left[ \delta j_\mathrm{\Omega} +  \delta u \,
        \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
        U_\tau \kappa \, y 
        \left(
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
       \right) 
          \right]  - 
             \delta k \left[  \frac{d \hat{k}}{dy} +\hat{\epsilon} \,  \frac{3 U_\tau }{2 \kappa y} +
             \frac{\sqrt{C_\mu}}{2} \,  \left(\frac{\mathrm{d} \hat u}{\mathrm{d} y}\right)
            \right] +
           \delta \epsilon \left[ \hat{\epsilon} \right]
           \right] \mathrm{d} y \, .
\end{align}
\begin{align}
    \hat{\epsilon} = 0 
    \quad \mathrm{and} \quad 
    \frac{d\hat{k}}{dy} = - \frac{\sqrt{C_\mu}}{2}  \left(\frac{\mathrm{d} \hat u}{\mathrm{d} y}\right)
    \qquad \rightarrow \qquad
    \int_y \left[ 
    \frac{\mathrm{d}}{\mathrm{d} y}  \left[ 
      \nu_t  \; 
        \frac{\mathrm{d} \hat u}{\mathrm{d} y} 
          \right] 
     \right] dy = 0 .
\end{align}

==> tex/scaling_derivation.tex <==
\section{Primal Scaling Analysis}
The laminar boundary-layer equations read:
\begin{alignat}{3}
R_\mathrm{1}^\mathrm{BL}:& v_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + v_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{1}{\rho} \frac{\partial p}{\partial x_\mathrm{1}}  - \frac{\partial}{\partial {x_\mathrm{2}}} \left[ \nu  \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} \right]  &&= 0 \\
R_\mathrm{2}^\mathrm{BL}:& \frac{1}{\rho} \frac{\partial p}{\partial x_\mathrm{2}}  &&= 0 \\
Q^\mathrm{BL}:&  -\frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{\partial v_\mathrm{2}}{\partial x_\mathrm{2}}  &&= 0.
\end{alignat}
Applying an Ensemble (Reynolds) averaging yields:
\begin{alignat}{3}
R_\mathrm{1}^\mathrm{BL,RA}:& \overline{v}_\mathrm{1} \frac{\partial \overline{v}_\mathrm{1}}{\partial x_\mathrm{1}} + \overline{v}_\mathrm{2} \frac{\partial \overline{v}_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{1}{\rho} \frac{\partial \overline{p}}{\partial x_\mathrm{1}}  - \frac{\partial}{\partial {x_\mathrm{2}}} \left[ \nu  \frac{\partial \overline{v}_\mathrm{1}}{\partial x_\mathrm{2}} \right] + \frac{1}{2} \frac{\partial \overline{v_\mathrm{1}^\prime v_\mathrm{1}^\prime}}{\partial x_\mathrm{1}}  + \frac{\partial \overline{v_\mathrm{2}^\prime v_\mathrm{1}^\prime}}{\partial x_\mathrm{2}} &&= 0 \\
R_\mathrm{2}^\mathrm{BL,RA}:& \frac{1}{\rho} \frac{\partial \overline{p}}{\partial x_\mathrm{2}}  &&= 0 \\
Q^\mathrm{BL,RA}:&  -\frac{\partial \overline{v}_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{\partial \overline{v}_\mathrm{2}}{\partial x_\mathrm{2}}  &&= 0.
\end{alignat}
The adjoint boundary layer equations follow from the Lagrangian:
\begin{align}
L = \int_\mathrm{\Gamma_\mathrm{O}} j_\mathrm{\Omega} \, \mathrm{d} \Gamma + \int_\mathrm{\Omega_\mathrm{O}} j_\mathrm{\Omega} \, \mathrm{d} \Omega  + \int_\mathrm{\Omega} \hat{v}_\mathrm{1} R_\mathrm{1}^\mathrm{BL} + \hat{v}_\mathrm{2} R_\mathrm{2}^\mathrm{BL} + \hat{p} Q^\mathrm{BL} \mathrm{d} \Omega.
\end{align}
First order optimality conditions force a vanishing Lagrangian in all dependent direction
\begin{align}
\delta_{\mathrm{v}_\mathrm{1}} L \cdot \delta v_\mathrm{1} &= ... + \int_\mathrm{\Omega} \delta v_\mathrm{1} \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} - v_\mathrm{1} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} - v_\mathrm{2} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial \hat{p}}{\partial x_\mathrm{1}} - \frac{\partial}{\partial {x_\mathrm{2}}} \left[ \nu  \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} \right] + \frac{\partial j_\mathrm{\Omega}}{\partial v_\mathrm{1}} \right] \mathrm{d} \Omega \\
\delta_{\mathrm{v}_\mathrm{2}} L \cdot \delta v_\mathrm{2} &= ... + \int_\mathrm{\Omega} \delta v_\mathrm{2} \left[ \hat{v}_\mathrm{2} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial \hat{p}}{\partial x_\mathrm{2}} + \frac{\partial j_\mathrm{\Omega}}{\partial v_\mathrm{2}} \right] \mathrm{d} \Omega \\
\delta_{p} L \cdot \delta p &= ... + \int_\mathrm{\Omega} \delta p \left[ \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} + \frac{\partial \hat{v}_\mathrm{2}}{\partial x_\mathrm{2}} + \frac{\partial j_\mathrm{\Omega}}{\partial p}  \right] \mathrm{d} \Omega.
\end{align}
Thus, the adjoint boundary-layer equations reads
\begin{alignat}{3}
\hat{R}_\mathrm{1}^\mathrm{BL}:& -v_\mathrm{1} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} - v_\mathrm{2} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} + \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} + \frac{\partial \hat{p}}{\partial x_\mathrm{1}} - \nu \frac{\partial^2 \hat{v}_\mathrm{1}}{\partial {x_\mathrm{2}}^2} &&= -\frac{\partial j_\mathrm{\Omega}}{\partial v_\mathrm{1}} \\
\hat{R}_\mathrm{2}^\mathrm{BL}:  & \; \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial \hat{p}}{\partial x_\mathrm{2}} &&= -\frac{\partial j_\mathrm{\Omega}}{\partial v_\mathrm{2}} \\
\hat{Q}^\mathrm{BL}:& - \frac{1}{\rho} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{1}{\rho}  \frac{\partial \hat{v}_\mathrm{2}}{\partial x_\mathrm{2}} &&= - \frac{\partial j_\mathrm{\Omega}}{\partial p}.
\end{alignat}
Applying an Ensemble (Reynolds) averaging on the adjoint boundary-layer equations yields:
\begin{alignat}{3}
\hat{R}_\mathrm{1}^\mathrm{BL,RA}:& -\overline{v}_\mathrm{1} \frac{\partial \overline{\hat{v}}_\mathrm{1}}{\partial x_\mathrm{1}} - \overline{v}_\mathrm{2} \frac{\partial \overline{\hat{v}}_\mathrm{1}}{\partial x_\mathrm{2}} + \overline{\hat{v}}_\mathrm{1} \frac{\partial \overline{v}_\mathrm{1}}{\partial x_\mathrm{1}} + \frac{\partial \overline{\hat{p}}}{\partial x_\mathrm{1}} - \nu \frac{\partial^2 \overline{\hat{v}}_\mathrm{1}}{\partial {x_\mathrm{2}}^2} - \frac{\partial \overline{v_\mathrm{1}^{\prime} \hat{v}_\mathrm{1}^{\prime}}}{\partial x_\mathrm{1}} - \frac{\partial \overline{v_\mathrm{2}^{\prime} \hat{v}_\mathrm{1}^{\prime}}}{\partial x_\mathrm{2}} + \overline{ \hat{v}_\mathrm{1}^{\prime} \frac{\partial v_\mathrm{1}^{\prime}}{\partial x_\mathrm{1}}} &&= -\frac{\partial j_\mathrm{\Omega}}{\partial \overline{v}_\mathrm{1}} \\
\hat{R}_\mathrm{2}^\mathrm{BL,RA}:  & \; \overline{\hat{v}}_\mathrm{1} \frac{\partial \overline{v}_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial \overline{\hat{p}}}{\partial x_\mathrm{2}} + \overline{ \hat{v}_\mathrm{1}^{\prime} \frac{\partial v_\mathrm{1}^{\prime}}{\partial x_\mathrm{2}}} &&= -\frac{\partial j_\mathrm{\Omega}}{\partial \overline{v}_\mathrm{2}} \\
\hat{Q}^\mathrm{BL,RA}:& - \frac{1}{\rho} \frac{\partial \overline{\hat{v}}_\mathrm{1}}{\partial x_\mathrm{1}} - \frac{1}{\rho}  \frac{\partial \overline{\hat{v}}_\mathrm{2}}{\partial x_\mathrm{2}} &&= - \frac{\partial j_\mathrm{\Omega}}{\partial p},
\end{alignat}
where we formally replaced the derivative of the objective w.r.t. the averaged field data. Alternative, we can define again a Lagrangian
\begin{align}
L = \int_\mathrm{\Gamma_\mathrm{O}} j_\mathrm{\Omega} \, \mathrm{d} \Gamma + \int_\mathrm{\Omega_\mathrm{O}} j_\mathrm{\Omega} \, \mathrm{d} \Omega  + \int_\mathrm{\Omega} \left[ \, \overline{\hat{v}}_\mathrm{1} + \hat{v}_\mathrm{1}^\prime \right] R_\mathrm{1}^\mathrm{BL,RA} + \left[ \, \overline{\hat{v}}_\mathrm{2} + \hat{v}_\mathrm{2}^\prime \right] R_\mathrm{2}^\mathrm{BL,RA} + \left[ \, \overline{\hat{p}} + \hat{p}^\prime \right] Q^\mathrm{BL,RA} \mathrm{d} \Omega,
\end{align}
where we need to compute necessary derivatives again, viz.
\begin{align}
\delta_{\overline{\mathrm{v}}_\mathrm{1}} L \cdot \delta \overline{v}_\mathrm{1} &= ... + \int_\mathrm{\Omega} \delta \overline{v}_\mathrm{1} \left[ \hat{v}_\mathrm{1} \frac{\partial v_\mathrm{1}}{\partial x_\mathrm{1}} - v_\mathrm{1} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{1}} - v_\mathrm{2} \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} + \frac{\partial \hat{p}}{\partial x_\mathrm{1}} - \frac{\partial}{\partial {x_\mathrm{2}}} \left[ \nu  \frac{\partial \hat{v}_\mathrm{1}}{\partial x_\mathrm{2}} \right] + \frac{\partial j_\mathrm{\Omega}}{\partial v_\mathrm{1}} \right] \mathrm{d} \Omega
\end{align}
